Personalizing ASR for Dysarthric and Accented Speech with Limited Data

Automatic speech recognition (ASR) systems have dramatically improved over the last few years. ASR systems are most often trained from 'typical' speech, which means that underrepresented groups don't experience the same level of improvement. In this paper, we present and evaluate finetuning techniques to improve ASR for users with non-standard speech. We focus on two types of non-standard speech: speech from people with amyotrophic lateral sclerosis (ALS) and accented speech. We train personalized models that achieve 62% and 35% relative WER improvement on these two groups, bringing the absolute WER for ALS speakers, on a test set of message bank phrases, down to 10% for mild dysarthria and 20% for more serious dysarthria. We show that 71% of the improvement comes from only 5 minutes of training data. Finetuning a particular subset of layers (with many fewer parameters) often gives better results than finetuning the entire model. This is the first step towards building state of the art ASR models for dysarthric speech.

==> sections/proposed_approach.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{sections/images/models.png}
  \label{fig:model_architecture}
  \caption{Schematic diagrams of the RNN-T architecture (left) and the LAS
    architecture (right). Diagrams come from \cite{Seq2SeqComparison2017}.}
\end{figure}

We create personalized ASR models by starting with a base model trained
on standard, unaccented speech. In order to verify that we are learning something other than
just the idiosyncrasies of a particular model, we run most of our experiments starting from
two different models: a Bidirectional RNN Transducer (RNN-T) model \cite{RNNT2012},
and a Listen, Attend, and Spell (LAS) model \cite{Chan2015}.
Both are end-to-end sequence-to-sequence models. We follow the training procedure
in \cite{Seq2SeqComparison2017} for the RNN-T model and \cite{CC2018} for the LAS model
(on the open source Librispeech dataset \cite{Librispeech}).

We finetune different layer combinations on different amounts of data, on both ALS and accents datasets. We
finetune models per speaker.

